SQN: Weakly-Supervised Semantic Segmentation of Large-Scale 3D Point Clouds

Labelling point clouds fully is highly time-consuming and costly. As larger point cloud datasets with billions of points become more common, we ask whether the full annotation is even necessary, demonstrating that existing baselines designed under a fully annotated assumption only degrade slightly even when faced with 1% random point annotations. However, beyond this point, e.g., at 0.1% annotations, segmentation accuracy is unacceptably low. We observe that, as point clouds are samples of the 3D world, the distribution of points in a local neighborhood is relatively homogeneous, exhibiting strong semantic similarity. Motivated by this, we propose a new weak supervision method to implicitly augment highly sparse supervision signals. Extensive experiments demonstrate the proposed Semantic Query Network (SQN) achieves promising performance on seven large-scale open datasets under weak supervision schemes, while requiring only 0.1% randomly annotated points for training, greatly reducing annotation cost and effort. The code is available at https://github.com/QingyongHu/SQN.

==> chapters/043_Network.tex <==
\smallskip\noindent\textbf{Implementation details.} \enskip
We use RandLA-Net \cite{hu2019randla} as the backbone of our framework due to its efficiency and the capacity to process large-scale point clouds. The hyperparameters including learning rate, optimizer, number of nearest neighbors keep the same for a fair comparison. We also follow \cite{xu2020weakly} to apply different data augmentation techniques on the input point clouds during training, including random flipping, random rotation, and random noise. 



